Decentralized Low-Rank State Estimation for Power Distribution Systems

This paper considers the low-observability state estimation problem in power distribution networks and develops a decentralized state estimation algorithm leveraging the matrix completion methodology. Matrix completion has been shown to be an effective technique in state estimation that exploits the low dimensionality of the power system measurements to recover missing information. This technique can utilize an approximate (linear) load flow model, or it can be used with no physical models in a network where no information about the topology or line admittance is available. The direct application of matrix completion algorithms requires solving a semi-definite programming (SDP) problem, which becomes infeasible for large networks. We therefore develop a decentralized algorithm that capitalizes on the popular proximal alternating direction method of multipliers (proximal ADMM). The method allows us to distribute the computation among different areas of the network, thus leading to a scalable algorithm. By doing all computations at individual control areas and only communicating with neighboring areas, the algorithm eliminates the need for data to be sent to a central processing unit and thus increases efficiency and contributes to the goal of autonomous control of distribution networks. We illustrate the advantages of the proposed algorithm numerically using standard IEEE test cases.

==> temp.tex <==
\begin{itemize}

\item 
\item Model free with some PMU Measurements
          \includegraphics[width=0.9 \columnwidth]{modelFree_16PMUs.jpg}

\item accuracy v number of PMUs for model free
      \includegraphics[width= \columnwidth]{MAPE_vs_NumberOfPMUs_ModelFree.jpg}

\item Full Model, no PMUs\\
      \includegraphics[width= \columnwidth]{november9_03.png}
\item showing that with full observability, it works better than just linear load flow model
      \includegraphics[width= \columnwidth]{fullVisibility_noPMU.jpg}

\item MAPE v fraction of data known
      \includegraphics[width= \columnwidth]{MAPE_vs_dataKnown.jpg}

\item Noise
\item MAPE v noise chart
\end{itemize}




\subsection{Convergence of Algorithm \ref{Agorthim:cenralAltMin}}
We start by presenting the following lemma bounding the norm of the iterates and $||\sum \langle A_i, U_iV_i^T\rangle -b_i||$.

\begin{lem}
Let $\{U_k\}$ and $\{V_k\}$ be the sequence of iterates generated by Algorithm \ref{Agorthim:cenralAltMin}.  Then, we have the following bounds.
\begin{equation}
\begin{aligned}
||U_k||_F^2 &\leq \alpha\\
||V_k||_F^2 &\leq \alpha\\
\sum|| \langle A_i, U_iV_i^T\rangle -b_i||& \leq \beta
\end{aligned}
\end{equation}
\end{lem}
\begin{proof}
Use the fact that 
\[||U^k|| \leq F(s^k) \leq F(s^0)\]
and 
\[\sum|| \langle A_i, U_iV_i^T\rangle -b_i|| \leq F(s^k) \leq F(s^0)\]
honestly does this deserve its own "lemma"?  idk
\end{proof}

Now, we can bound the gradient of $F(s^k)$ by the norm difference of the iterates $||s^k-s^{k-1}||$.  
\begin{lem}
There exists a constant $w$ such that 
\begin{equation}
\label{lemma1}
    ||\nabla F(s^{k+1})||_F \leq w ||s^{k+1}-s^{k}||_F 
\end{equation}
\end{lem}
\begin{proof}
Clearly by first order necessary condition of the subproblem for $V_k$, we have that $\nabla _V F(U^{k+1}, V^{k+1})=0$.  Now, to bound $\nabla _U F(U^{k+1}, V^{k+1})$, we start by observing that, by first order necessary condition of the $U$ subproblem, \begin{equation}
\label{USubProbDerivIs0}
    \begin{aligned}
    U^{k+1}+\sum (\langle A_i, U^{k+1}V^{k}\rangle-b_i)A_i V^{k}=0
    \end{aligned}
\end{equation}
Now, we have 
\begin{equation*}
    \begin{aligned}
    \nabla &_U F(s^{k+1})=U^{k+1}+\sum (\langle A_i, U^{k+1}V^{k+1}\rangle-b_i)A_i V^{k+1}\\
    =&U^{k+1}+\sum (\langle A_i, U^{k+1}V^{k+1}\rangle-b_i)A_i V^{k+1}\\
    &-(U^{k+1}+\sum (\langle A_i, U^{k+1}V^{k}\rangle-b_i)A_i V^{k})\\
    =&(\sum -b_i A^i) (V^{k+1}-V^k)) +\sum \langle U^{k+1}^TA_i, V^{k+1}\rangle A_i V^{k+1}\\
    & -\sum \langle U^{k+1}^TA_i, V^{k}\rangle A_i V^{k}\\
    =&(\sum -b_i A^i) (V^{k+1}-V^k)) +\sum \langle U^{k+1}^TA_i, V^{k+1}\rangle) A_i V^{k+1}\\
    & -(\sum \langle U^{k+1}^TA_i, V^{k+1}\rangle+\sum \langle U^{k+1}^TA_i, V^{k}-V^{k+1}\rangle) A_i V^{k}\\
    =&\sum ( \langle A_i, U^{k+1}V^{k+1}^T\rangle-b_i)A_i (V^{k+1}-V^k)\\
    &+\sum \langle U^{k+1}^T A_i, V^k-V^{k+1}\rangle A_i V^k
    \end{aligned}
\end{equation*}
The first step is the definition of $F$, and the second uses equation (\ref{USubProbDerivIs0}).  We can now bound $||\nabla_U F(s^{k+1})||$.
\begin{equation*}
    \begin{aligned}
    ||\nabla_U F(s^{k+1})||&\leq\sum ||\langle A_i, U^{k+1}V^{k+1}^T \rangle-b_i ||_F ||A_i||_F ||V^{k+1} -V^k||\\ 
    &+\sum ||\langle U^{k+1}^T A_i, V^{k+1}-V^k\rangle A_i V^k||\\
    \leq &\alpha(\sum ||A_i||)||V^{k+1} -V^k||\\
    &+ \beta (\sum ||A_i||) ||V^{k+1} -V^k||\\
     \leq& w ||s^{k+1}-s^k||_F^2
    \end{aligned}
\end{equation*}
Thus we have shown. (\ref{lemma1})
\end{proof}
We can now prove Theorem \ref{centralizedAlgorithmConvergence}.
\begin{proof}
\begin{equation*}
    \begin{aligned}
F(U^{k+1}, V^{k+1}) \leq &F(U^{k+1}, V^{k}) -\frac{\mu}{2} ||V^{k+1}-V^k||_F^2\\
\leq& F(U^{k}, V^{k}) -\frac{\mu}{2} ||V^{k+1}-V^k||_F^2\\ &-\frac{\mu}{2} ||U^{k+1}-U^k||_F^2\\
= &F(U^{k}, V^{k}) -\frac{\mu}{2} ||s^{k+1}-s^k||_F^2
\end{aligned}
\end{equation*}
Where both steps make use of the $\mu$ strong convexity of the objective in each variable.  Rearranging the inequality and summing over all $k$, we get
\begin{equation*}
    \begin{aligned}
    \sum_{k=0}^\infty F(s^k)-F(s^{k+1}) &\geq \frac{\mu}{2}\sum_{k=0}^\infty ||s^{k+1}-s^k||_F^2\\
    F(s^0) &\geq \frac{\mu}{2}\sum_{k=0}^\infty ||s^{k+1}-s^k||_F^2
    \end{aligned}
\end{equation*}
Which is to say, $$\lim_{k \rightarrow \infty}||s^{k+1}-s^{k}||=0$$ 
Thus showing the asymptotic convergence of $\{ s^k \}_k$.  Using Equation (\ref{lemma1}), we have that 
\begin{equation*}
    \lim_{k \rightarrow \infty} \nabla F(s^k) \leq \lim_{k \rightarrow \infty}||s^{k+1}-s^{k}||=0
\end{equation*}
Which shows that any limit point of the sequence of iterates satisfies the first order necessary condition for optimally. 
\end{proof}

